Multi-contact MPC for Dynamic Loco-manipulation on Humanoid Robots

This paper presents a novel method to control humanoid robot dynamic loco-manipulation with multiple contact modes via multi-contact Model Predictive Control (MPC) framework. The proposed framework includes a multi-contact dynamics model capable of capturing various contact modes in loco-manipulation, such as hand-object contact and foot-ground contacts. Our proposed dynamics model represents the object dynamics as an external force acting on the system, which simplifies the model and makes it feasible for solving the MPC problem. In numerical validations, our multi-contact MPC framework only needs contact timings of each task and desired states to give MPC the knowledge of changes in contact modes in the prediction horizons in loco-manipulation. The proposed framework can control the humanoid robot to complete multi-tasks dynamic loco-manipulation applications such as efficiently picking up and dropping off objects while turning and walking.

==> Commands.tex <==
%!TEX root = ../Main.tex
% Defines commands to easily input variables and equations into the paper.

% Matrix commands for simple matrices
\newcommand{\pMat}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\bMat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\BMat}[1]{\begin{Bmatrix}#1\end{Bmatrix}}
\newcommand{\aMat}[1]{\begin{Vmatrix}#1\end{Vmatrix}}
\newcommand{\mat}[1]{\begin{matrix}#1\end{matrix}}

% Pat commands
\newcommand{\cross}[1]{ {[#1]}_{\times} }

% Reference Frames
\newcommand{\IFrame}{\mathcal{I}}
\newcommand{\BFrame}{\mathcal{B}}
\newcommand{\COM}{CoM}

% State definitions
\newcommand{\roll}{\theta}
\newcommand{\pitch}{\phi}
\newcommand{\yaw}{\psi}

\newcommand{\rollhat}{\hat{\theta}}
\newcommand{\pitchhat}{\hat{\phi}}
\newcommand{\yawhat}{\hat{\psi}}



\newcommand{\dRoll}{\dot{\roll}}
\newcommand{\dPitch}{\dot{\pitch}}
\newcommand{\dYaw}{\dot{\yaw}}

\newcommand{\omegaX}{\omega_x}
\newcommand{\omegaY}{\omega_y}
\newcommand{\omegaZ}{\omega_z}

\newcommand{\dX}{\dot{x}}
\newcommand{\dY}{\dot{y}}
\newcommand{\dZ}{\dot{z}}

\newcommand{\quat}{\bm{q}}
\newcommand{\pos}{\bm{p}}
\newcommand{\angVel}{\bm{\omega}}
\newcommand{\vel}{\bm{v}}
\newcommand{\posDot}{\bm{\dot{\pos}}}
\newcommand{\posDotDot}{\bm{\ddot{p}}}
\newcommand{\quatDot}{\bm{\dot{\quat}}}
\newcommand{\angVelDot}{\bm{\dot{\angVel}}}

% Desired Variables
\newcommand{\xd}{\bm{x}_d}
\newcommand{\uref}{\bm{u}_{ref}}

% State component vectors
\newcommand{\quatV}{q_0 \\ q_x \\ q_y \\ q_z}
\newcommand{\quatVector}{\BMat{\quatV}}
\newcommand{\posV}{x \\ y \\ z}
\newcommand{\posVector}{\BMat{\posV}}
\newcommand{\angVelV}{\omegaX \\ \omegaY \\ \omegaZ}
\newcommand{\angVelVector}{\BMat{\angVelV}}
\newcommand{\velV}{\dX \\ \dY \\ \dZ}
\newcommand{\velVector}{\BMat{\velV}}

\newcommand{\rpyV}{\roll \\ \pitch \\ \yaw}
\newcommand{\rpyVector}{\BMat{\rpyV}}
\newcommand{\rpyDotV}{\dRoll \\ \dPitch \\ \dYaw}
\newcommand{\rpyDotVector}{\BMat{\rpyDotV}}

% Parameter Estimates
\newcommand{\state}{\bm{x}}
\newcommand{\stateDot}{\bm{\dot{\state}}}
\newcommand{\stateEstimate}{\bm{\hat{x}}}
\newcommand{\rFootEstimate}{\bm{\hat{r}}}
\newcommand{\forceEstimate}{\bm{\hat{F}}}
\newcommand{\rFootEstimatef}{\bm{\hat{r}}_f}
\newcommand{\forceEstimatef}{\bm{\hat{F}}_f}
\newcommand{\inputU}{\bm{u}}
\newcommand{\inputEstimate}{\bm{\hat{u}}}
\newcommand{\outputEstimate}{\bm{\hat{y}}}

% State and Input Vectors
\newcommand{\stateVector}{\BMat{\posV \\ \quatV \\ \velV \\ \angVelV}}
\newcommand{\stateVectorRed}{\BMat{\posV \\ \rpyV \\ \velV \\ \rpyDotV}}
\newcommand{\inputVector}{\BMat{\rFootEstimate_1 \\ \forceEstimate_1 \\ \rFootEstimate_2 \\ \forceEstimate_2 \\ \rFootEstimate_3 \\ \forceEstimate_3 \\ \rFootEstimate_4 \\ \forceEstimate_4}}

% Variable Transformations
\newcommand{\quatToRPY}{\bMat{\tan^{-1}\pMat{\dfrac{2\pMat{q_0q_1+q_2q_3}}{1-2\pMat{q_1^2+q_2^2}}}\\ \sin^{-1}\pMat{2\pMat{q_0q_2+q_3q_1}} \\ \tan^{-1}\pMat{\dfrac{2\pMat{q_0q_3+q_1q_2}}{1-2\pMat{q_2^2+q_3^2}}}}}
\newcommand{\omegaToRPYDot}{\bMat{\dfrac{\cos\pMat{\yaw}}{\cos\pMat{\pitch}} & \dfrac{\sin\pMat{\yaw}}{\cos\pMat{\pitch}} & 0 \\ -\sin\pMat{\yaw} & \cos\pMat{\yaw} & 0 \\ \dfrac{\cos\pMat{\yaw}\sin\pMat{\pitch}}{\cos\pMat{\pitch}} & \dfrac{\sin\pMat{\yaw}\sin\pMat{\pitch}}{\cos\pMat{\pitch}} & 1}}

% Time step definitions
\newcommand{\n}[1]{#1_n}
\renewcommand{\k}[1]{#1_k}
\newcommand{\nk}[1]{#1_{i}}

% Decision Variables Full
\newcommand{\inputVarsV}{\rFootEstimate \\ \forceEstimate}
\newcommand{\inputVarsVectorf}[1]{\BMat{\inputVarsV}_#1}
\newcommand{\decisionVarsVFull}{\inputVarsVectorf{1} \\ \vdots \\ \inputVarsVectorf{4} \\ \stateEstimate}
\newcommand{\decisionVarsVectorFull}[2]{\BMat{\decisionVarsVFull}_{#1,#2}}
\newcommand{\decisionArrayVFull}{\decisionVarsVectorFull{1}{1} & \hdots & \decisionVarsVectorFull{1}{K_1} & \hdots & \decisionVarsVectorFull{N}{1} & \hdots & \decisionVarsVectorFull{N}{K_N}}
\newcommand{\decisionArrayVectorFull}{\bMat{\decisionArrayVFull}}

% Decision Variables 
\newcommand{\decisionVarsV}{\stateEstimate \\ \inputEstimate}
\newcommand{\decisionVarsVector}{\BMat{\decisionVarsV}}
\newcommand{\decisionArrayV}{\decisionVarsVector_{1,1} & \hdots & \decisionVarsVector_{N,K_N}}
\newcommand{\decisionArrayVector}{\bMat{\decisionArrayV}}

% Simple Dynamics
\newcommand{\forces}{\bm{f}}
\newcommand{\torques}{\bm{\tau}}
\newcommand{\forceIEstimate}{\phantom{{}^\IFrame}\bm{\hat{f}}}
\newcommand{\torquesBEstimate}{^\BFrame\bm{\hat{\tau}}}
\newcommand{\RMatItoB}{^\BFrame\mathbf{R}_\IFrame}
\newcommand{\RMatItoBEstimate}{^\BFrame\mathbf{\hat{R}}_\IFrame}
\newcommand{\RMatBtoI}{^\IFrame\mathbf{R}_\BFrame}
\newcommand{\inputForceTorqueFunction}{ \hat{h}\!\pMat{\nk{\stateEstimate}, \nk{\inputEstimate}}}
\newcommand{\inputForceTorque}{\BMat{\phantom{{}^\BFrame}\forces \\ {}^\BFrame\torques}}
\newcommand{\inputForceTorqueMPC}{\BMat{\forceIEstimate \\ \torquesBEstimate}}
\newcommand{\forceTorqueTransform}{\bMat{\mathbf{I} & 0 \\ 0 & {\bm{R}_z^T(\yawhat)}}}
\newcommand{\uToForceTorqueMat}{\bMat{\mat{\mathbf{I} \\ \bMat{\bm{r}_1}_\times} & \hdots & \mat{\mathbf{I} \\ \bMat{\bm{r}_f}_\times}}}
\newcommand{\uToForceTorqueMatEstimate}{\bMat{\mat{\mathbf{I} \\ \bMat{\rFootEstimate_1}_\times} & \hdots & \mat{\mathbf{I} \\ \bMat{\rFootEstimate_f}_\times}}}
% Equation
\newcommand{\AMatnk}{{\bm{A}}_i}
\newcommand{\BMatnk}{{\bm{B}}_i}
\newcommand{\simpleDynamicsEq}{\AMatnk\nk{\stateEstimate}+\BMatnk\inputForceTorqueFunction+\bm{d}_i}
\newcommand{\simpleDynamics}{\stateEstimate_{i+1}=\simpleDynamicsEq}
% Matrix Linear
\newcommand{\AMatFull}{\bMat{\mathbf{I}_6 & \Delta t_i\mathbf{I}_6 \\ 0 & \mathbf{I}_6}}
\newcommand{\BMatFull}{\bMat{\frac{\Delta t_i^2}{2} \,{}^{\BFrame}\!\bm{I}^{-1} \\[.75ex] \Delta t_i\, {}^{\BFrame}\!\bm{I}^{-1} }}

\newcommand{\BMatFcull}{\bMat{\bMat{\frac{dt_n^2}{2}\mathbf{I}_6 \\ dt_n\mathbf{I}_6}\bMat{\frac{1}{m}\mathbf{I}_3 & 0 \\ 0 & ^\BFrame\bm{I}^{-1}}}}
	
	
	
% Full Dynamics
\newcommand{\sumForces}{\sum^\IFrame\bm{F}}
\newcommand{\sumTorques}{\sum^\IFrame\bm{\tau}}
\newcommand{\stateReducedVector}{\BMat{\pos \\ {}^\IFrame\!\bm{R}_{\BFrame} \\ \posDot \\ \angVel}}

\newcommand{\dynamicsReducedVector}{\BMat{
\posDot_c \\[.5ex]
{}^\IFrame\!\bm{R}_{\BFrame} \left[ {}^\BFrame \angVel\right]_\times \\[.5ex] 
\frac{1}{m}\forces - \bm{g} \\[.5ex]  
{}^\BFrame\,\overline{\!\bm{I}}{}^{-1}\pMat{{}^\BFrame\torques - {}^\BFrame \angVel\times {{}^\BFrame\,\overline{\!\bm{I}}}\,\,{\vphantom{\bm{I}}}^\BFrame\angVel}
}}


\newcommand{\stateDotReducedVector}{\BMat{\posDot_c \\ {}^\IFrame\!\dot{\bm{R}}_{\BFrame} \\ \posDotDot_c \\ {}^\BFrame\angVelDot}}

% Reference Input
\newcommand{\KPercent}{K_\%}
\newcommand{\pFootRef}{\bm{p}_{ref,f,xy,k} = \bm{\hat{p}}_{h,xy} + \posDot_{d,xy}T_{s}\pMat{\frac{1}{2}-\KPercent}+\\\pMat{\bm{\dot{\hat{p}}}_{xy} -\posDot_{d,xy}}\sqrt{\frac{\hat{p}_z}{\aMat{\bm{g}}}}\pMat{1 - \KPercent}}
			
% Error definitions
\newcommand{\stateError}{\bm{\tilde{x}}}
\newcommand{\inputError}{\bm{\tilde{u}}}
\newcommand{\stateErrorFull}{\xd-\outputEstimate}
\newcommand{\inputErrorFull}{\uref-\inputEstimate}
			
% Basic Cost Function
\newcommand{\basicArgs}{\stateEstimate, \hat{\bm{u}}}
\newcommand{\basicMin}{\underset{\basicArgs}{\text{min}}}
\newcommand{\basicCost}{J\pMat{\basicArgs}}
\newcommand{\basicCostFunction}{\basicMin\basicCost}
			
% MPC Function
\newcommand{\MPCSum}{\sum\limits_{n=1}^{N}\sum\limits_{k=1}^{\n{K}}}
%\newcommand{\MPCMin}{\underset{\stateEstimate, \inputEstimate}{\text{min}}}
\newcommand{\MPCMin}{\underset{\chi}{\text{min}}}
\newcommand{\stateCost}{\stateError^T\bm{Q}\stateError}
\newcommand{\inputCost}{\inputError^T\bm{R}\inputError}
\newcommand{\MPCCost}{\stateCost+\inputCost}
\newcommand{\MPCCostFunction}{\MPCMin\MPCSum\pMat{\MPCCost}_{n,k}}
			
% MPC Function Full
\newcommand{\MPCMinFull}{\underset{\stateEstimate, \inputEstimate}{\text{min}}}
\newcommand{\stateCostFull}{\pMat{\stateErrorFull}^T\bm{Q}\pMat{\stateErrorFull}}
\newcommand{\inputCostFull}{\pMat{\inputErrorFull}^T\bm{R}\pMat{\inputErrorFull}}
\newcommand{\MPCCostFull}{\stateCostFull+\inputCostFull}
\newcommand{\MPCCostFunctionFull}{\MPCMinFull\MPCSum\pMat{\MPCCostFull}_{n,k}}
			
% Constraints
\newcommand{\dynamicsConstraint}{\stateEstimate_{nk+1}=\simpleDynamicsEq}
\newcommand{\groundConstraint}{p_{z,f}=\hat{z}_g \pMat{p_{x,f}, p_{y,f}}}
\newcommand{\kinematicLegConstraint}{\aMat{\bm{r}_{h \to f}} \leq l_{f,max}}
\newcommand{\slipConstraint}{\bm{p}_{f,k+1} = \bm{p}_{f,k}}
\newcommand{\frictionConstraint}[1]{{-}\mu\bm{F}_{z,f}\leq\bm{F}_{#1,f}\leq\mu\bm{F}_{z,f}}
\newcommand{\frictionConeConstraint}{\frictionConstraint{x} \\ \frictionConstraint{y}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CONTACT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\legState}{s}
\newcommand{\legStateScheduled}{\legState_{\phi}}
\newcommand{\legStateNotScheduled}{\bar{\legState}_{\phi}}
\newcommand{\legStateEstimated}{\hat{\legState}}
\newcommand{\contactState}{c}
\newcommand{\swingState}{\bar{\contactState}}
\newcommand{\contactStateScheduled}{\contactState_{\phi}}
\newcommand{\swingStateScheduled}{\bar{\contactState}_{\phi}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Support Polygon
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\phaseGain}{\Phi}
\newcommand{\adjLegP}{^{+}}
\newcommand{\adjLegM}{^{-}}

==> Sections/Control.tex <==
\section{Contact-schedule-based Control}
\label{sec:Control}

In this section, we present the contact-schedule-based control framework for synchronized humanoid loco-manipulation. In detail, we present the hybrid control framework including CSMPC and CSWBC. 

\subsection{Contact Schedule Visualization}
\label{subsec:contactSchedule}

The contact schedule in MPC is very powerful due to the predictive nature of MPC that optimizes the current control input by the knowledge of future dynamic changes. We leverage this to allow robots to have frequent changes in dynamics. A visualization of the contact schedule in CSMPC is shown in Figure. \ref{fig:contactSchedule}. This contact schedule describes a task commanding the robot to pick-up and walk with an object. 



\subsection{CSMPC Formulation}
\label{subsec:CSMPC_form}

First, we present the CSMPC formulation that employs the SRBD proposed in Section.\ref{subsec:CSMPC}. We choose the state variables as $[{\bm \Theta};{\bm p}_c;{\bm \omega};\dot {{\bm p}}_c]$ and control inputs as $\bm U= [\bm u; \bm F_{ext}]$, then the simplified dynamics equation can be represented as
\begin{align}
\label{eq:simpDyn}
\frac{d}{dt}\left[\begin{array}{c} {\bm \Theta}\\{\bm p}_c\\{\bm \omega}\\\dot {{\bm p}}_c \end{array} \right] 
= \bm A \left[\begin{array}{c} {\bm \Theta}\\{\bm p}_c\\{\bm \omega}\\\dot {{\bm p}}_c \end{array} \right] + \bm B \bm U + \left[\begin{array}{c} 0\\0\\0\\\bm g \end{array} \right] 
\end{align}

\begin{align}
\label{eq:A}
\bm A = \left[\begin{array}{cccc} 
\mathbf 0_3 & \mathbf 0_3 & \mathbf R_b^{-1} & \mathbf 0_3 \\
\mathbf 0_3 & \mathbf 0_3 & \mathbf 0_3 & \mathbf I_3\\
\mathbf 0_3 & \mathbf 0_3 & \mathbf 0_3 & \mathbf 0_3\\
\mathbf 0_3 & \mathbf 0_3 & \mathbf 0_3 & \mathbf 0_3 \end{array} \right], 
\mathbf R_b = \left[\begin{array}{ccc}
{c_\theta}{c_\psi} & -{s_\psi} & 0 \\
{c_\theta}{s_\psi} & c_\psi & 0 \\
-s_\theta & 0 & 1  \end{array} \right] 
\end{align}

\begin{align}
\label{eq:B}
\bm B = \left[\begin{array}{ccccc} 
\mathbf 0_3 & \mathbf 0_3 & \mathbf 0_{3\times2} & \mathbf 0_{3\times2} & \mathbf 0_3\\
\mathbf 0_3 & \mathbf 0_3 & \mathbf 0_{3\times2} & \mathbf 0_{3\times2}  & \mathbf 0_3 \\ 
\frac{\sigma _{C1} \bm r_1\times}{\bm I_G}  & \frac{\sigma _{C2} \bm r_2\times}{\bm I_G} & 
\frac{\sigma _{C1}\mathbf L}{\bm I_G}   & \frac{\sigma _{C2} \mathbf L}{\bm I_G} & \frac{\sigma _{e}\bm r_e\times}{\bm I_G}\\
\frac{\sigma _{C1}\mathbf {I}_{3}}{m_{ub}}  & \frac{\sigma _{C2} \mathbf {I}_{3}}{m_{ub}} &  \mathbf {0}_{3\times2} &  \mathbf {0}_{3\times2} & \frac{\sigma _{e}\mathbf {I}_{3}}{m_{ub}} \end{array}  \right]
\end{align}
where $s$ denotes sine operator and $c$ denotes cosine operator. Note that $\mathbf R_b$ is not inevitable at $\theta = \pm90^\circ$. We intend to not allow the robot to have a pitch angle of $\pm90^\circ$ in any tasks.

To guarantee the linear relation in the formulation of Equation (\ref{eq:simpDyn}), we choose to include gravity $\bm g \in \mathbb{R}^3$ as a dummy variable in  decision variables $\bm x = [{\bm \Theta};{\bm p}_c;{\bm \omega};\dot {{\bm p}}_c; \bm g]\in \mathbb{R}^{15}$, to form a state-space equation, with continuous-time matrices ${\hat{\bm A_c}}$ and ${\hat{\bm B_c}}$: 
\begin{align}
\label{eq:linearSS}
\dot{{\bm { x}}}(t) =  {\hat{\bm A_c}} {{\bm {x}}} +  {\hat{\bm B_c}} \bm U.
\end{align}

 The formulation of the MPC problem with finite horizon $k$ is written as follows. The objective of the problem is to drive state $\bm x$ close to the desired input while minimizing $\bm U$. The desired input, mentioned in Section. \ref{sec:dynamicsModel}, are hybrid rigid body state information (i.e. body leans backwards). These objectives are weighted by matrices $\bm Q_i$ and $\bm R_i$.
\begin{align}
\label{eq:MPCform}
%\nonumber
\underset{\bm{x,U}}{\operatorname{min}}   \:\:  & \sum_{i = 0}^{k-1}(\bm x_{i+1}-  \bm x_{i+1}^{ref})^T\bm Q_i(\bm x_{i+1}- \bm x_{i+1}^{ref}) + \bm{R}_i\| \bm{U}_i \|
\end{align}
%%
\begin{subequations}
\begin{align}
\label{eq:dynamicCons}
\:\:\operatorname{s.t.} \quad  {\bm {x}}[i+1] = \bm {\hat{A}}[i]\bm x[i] + \bm {\hat{B}}[i]\bm U[i], \\
\label{eq:frictionCons}
\nonumber 
-\mu  {F}_{nz} \leq  F_{nx} \leq \mu {F}_{nz} \quad \quad\\
-\mu {F}_{nz} \leq  F_{ny} \leq \mu {F}_{nz} \quad \quad\\
\label{eq:forceCons}
0<  {F}_{min} \leq  F_{nz} \leq  {F}_{max} \quad \quad\\
\label{eq:forceCons2}
\bm {F}_{ext} =  \left[\begin{array}{ccc} 0 & 0 & m_og \end{array} \right]^\intercal \quad \quad
\end{align}
\end{subequations}

Equation (\ref{eq:dynamicCons}) to (\ref{eq:forceCons}) are constraints of the MPC problem. Equation (\ref{eq:dynamicCons}) is an equality constraint of the linearized dynamics equation in discrete-time at $i$th time-step derived from equation (\ref{eq:linearSS}). Equation (\ref{eq:frictionCons}) describes inequality constraints on contact friction pyramid. Equation (\ref{eq:forceCons}) describes the bounds of reaction forces. Equation (\ref{eq:forceCons2}) is an equality constraint that ensures the external force from control input is equal to gravitational force of the object.

The translation of the proposed MPC problem into Quadratic Programming (QP) form to be efficiently solved can be found in many related works and previous works (e.g., \cite{di2018dynamic}, \cite{li2021force}).

\begin{figure}[!t]
\vspace{0.2cm}
		\center
		\includegraphics[clip, trim=7cm 1.3cm 10cm 8.5cm, width=\columnwidth]{Figures/contactSchedule.pdf}
		\caption{{\bfseries MPC Contact Schedule Visualized} }
		\label{fig:contactSchedule}
		\vspace{-0.4cm}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Task-oriented Cartesian PD Control}
\label{subsec:CartesianPD}

While the CSMPC primarily provides optimal ground reaction force-and-moments to the stance legs during locomotion, we choose to use Cartesian-space PD control to manipulate arms and swing foot $n$ based on the tasks and contact schedules. The desired swing foot location $\bm p_{f,n}^{des} \in \mathbb R^{3}$ follows a heuristic foot placement policy based on spring-loaded inverted pendulum \cite{raibert1986legged}, with addition of the consideration of desired CoM linear speed, $\dot{\bm p}_c^{des}$ \cite{kim2019highly},
\begin{align}
\label{eq:footPlacement}
\bm p_{f,n}^{des} =  \bm p_{c} + \dot{\bm p}_c \Delta t/2 + k(\dot{\bm p}_c-\dot{\bm p}_c^{des}),
\end{align}
where $\Delta t$ is the gait period and $k$ is a scaling factor for tracking desired linear velocity. (e.g., push-recovery)

The $n$th swing foot force by Cartesian PD control is 
\begin{align}
\label{eq:pdlaw}
\bm F_{swing,n}=\bm K_P(\bm p_{f,n}^{des}-\bm p_{f,n})+\bm K_D(\dot{\bm p}_{f,n}^{des}-\dot{\bm p}_{f,n})
\end{align}

Similarly, to control the $m$th hand of the robot to move to desired task locations $\bm p_{h,m}^{des} \in \mathbb R^{3}$, the hand force is 
\begin{align}
\label{eq:pdlaw2}
\bm F_{hand,m}=\bm K_P(\bm p_{h,1}^{des}-\bm p_{h,m})+\bm K_D(\dot{\bm p}_{h,m}^{des}-\dot{\bm p}_{h,m})
\end{align}

%%%%%%%%%%
\begin{figure*}[!t]
	\vspace{0.2cm}
    \center
    \includegraphics[width=\textwidth]{Figures/snapshots.png}
    \caption{{\bfseries Simulation Snapshots} Simulation snapshots of 1) Pickup, walk, and drop off a 4 $\unit{kg}$ box object, 2) Pickup, walk in place, and throw a 2 $\unit{kg}$ spherical object. Blue region represents the origin of the object. Orange region represents the target local for drop-off. }
    \label{fig:snapshots}
    \vspace{-0.7cm}
\end{figure*}

%%%%%%%%%%

\subsection{CSWBC Formulation}
\label{subsec:CSWBC_form}

To synchronize the hybrid controller inputs from Section. \ref{subsec:CSMPC_form} to \ref{subsec:CartesianPD} and leverage the whole-body dynamics model in Section. \ref{subsec:CSWBC}, we use a contact-schedule-based WBC to collect all control inputs and solve for optimal joint torques. The CSWBC is simplified and formed into a QP problem for efficient execution and high frequency. The desired command in CSWBC is based on the desired states of the robot $\bm x_c^{des} = [\bm p_c^{des}; \bm \Theta^{des}]$, by a simple PD control law:
\begin{align}
\label{eq:desAcc}
\ddot{\bm x}_c^{des} = \bm K_p(\bm x_c^{des} - \bm x_c) + \bm K_d(\dot{\bm x}_c^{des} - \dot{\bm x}_c)
\end{align}

The desired acceleration command $\bm \ddot{x}_c^{des}$ is translated into task-space $\ddot {\mathbf {q}}_{cmd}$ by an inverse-kinematic-based null space projection technique described in \cite{kim2019highly}. 

Now the WBC-QP problem to compute the minimized relaxation components of MPC ground reaction force $\Delta \bm u$ and joint acceleration command $\Delta \ddot{\mathbf q}$ is as follows,
\begin{align}
\label{eq:WBC-QP}
%\nonumber
\underset{{\Delta \ddot{\mathbf q},\Delta \bm u}}{\operatorname{min}}   \:\:  & 
\Delta \ddot{\mathbf q}^\intercal {\mathbf H} \Delta \ddot{\mathbf q} + \Delta \bm u^\intercal {\mathbf K} \Delta \bm u
\vspace{0.5cm}
\end{align}
\begin{subequations}
\begin{align}
\label{eq:WBC_cons1}
\nonumber
\operatorname{s.t.} \quad 
\mathbf S_{b}\{\mathbf M (\Delta \ddot{\mathbf q} + \ddot{\mathbf q}_{cmd}) + \mathbf C + \mathbf g \\ 
- \bm \tau_f(t, \Delta \bm u , \bm u)\} = \mathbf 0 \\
\label{eq:WBC_cons3}
\quad  \quad  \quad  \bm u_{min} \leq \Delta \bm u + \bm u \leq \bm u_{max} \quad\\
\label{eq:WBC_cons4}
\quad  \quad  \quad  \bm \tau_{min} \leq \bm \tau \leq \bm \tau_{max} \quad
\end{align}
\end{subequations}

In equation (\ref{eq:WBC-QP}), $\mathbf H \in  \mathbb{R}^{16\times16}$ and $\mathbf K \in  \mathbb{R}^{10\times10}$ are diagonal weighting matrices for each objective. Equation (\ref{eq:WBC_cons1}) is a dynamics constraint formed by equation \ref{eq:EOM1} in order to control the floating base dynamics. Selection matrix $\mathbf S_{b}$ consists of 1s and 0s to identify the float base joints.

Finally, the optimal joint torque $\bm \tau$ can be calculated as
\begin{align}
\label{eq:torque}
\left[\begin{array}{c}  \bm 0 \\  \bm \tau \end{array} \right] 
= \mathbf M (\Delta \ddot{\mathbf q} + \ddot{\mathbf q}_{cmd}) + \mathbf C + \mathbf g - \bm \tau_f(t, \Delta \bm u , \bm u)
\end{align}

where $\bm \tau_f$ is a time-dependent term that summarizes all external forces applied to the system based on the contact schedules, shown in equation \ref{eq:EOM2}. The swing foot and hand forces are feed-forward from Cartesian PD controller, and optimal reaction force-and-moments are $\Delta \bm u+\bm u$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

